Semi-Streaming Algorithms for Annotated Graph Streams

Considerable effort has been devoted to the development of streaming algorithms for analyzing massive graphs. Unfortunately, many results have been negative, establishing that a wide variety of problems require $\Omega(n^2)$ space to solve. One of the few bright spots has been the development of semi-streaming algorithms for a handful of graph problems -- these algorithms use space $O(n\cdot\text{polylog}(n))$. In the annotated data streaming model of Chakrabarti et al., a computationally limited client wants to compute some property of a massive input, but lacks the resources to store even a small fraction of the input, and hence cannot perform the desired computation locally. The client therefore accesses a powerful but untrusted service provider, who not only performs the requested computation, but also proves that the answer is correct. We put forth the notion of semi-streaming algorithms for annotated graph streams (semi-streaming annotation schemes for short). These are protocols in which both the client's space usage and the length of the proof are $O(n \cdot \text{polylog}(n))$. We give evidence that semi-streaming annotation schemes represent a substantially more robust solution concept than does the standard semi-streaming model. On the positive side, we give semi-streaming annotation schemes for two dynamic graph problems that are intractable in the standard model: (exactly) counting triangles, and (exactly) computing maximum matchings. The former scheme answers a question of Cormode. On the negative side, we identify for the first time two natural graph problems (connectivity and bipartiteness in a certain edge update model) that can be solved in the standard semi-streaming model, but cannot be solved by annotation schemes of "sub-semi-streaming" cost. That is, these problems are just as hard in the annotations model as they are in the standard model.

==> prelims.tex <==
\section{Preliminaries}

\subsection{Data Stream Models}\label{full::sec:streammodel}

We now define our annotated data stream models.  Recall that a (traditional)
data stream algorithm computes a function $\fn$ of an input sequence
$\bx \in\universe^\length$, where $\length$ is the number of stream updates, and $\universe$ is some data universe, such as 
$\b^b$
or
$[n] = \{0, \dots, n-1\}$: the algorithm uses a limited amount of working memory and has
access to a random string. The function $\fn$ may or may not be Boolean.
%When it is not, we may permit an approximate answer: we accept any answer in the set $C(f(\bx))$, for some function $C$. 

An annotated data stream algorithm, or a {\em \ascheme}, is a pair $\alg =
(\help,V)$, consisting of a help function $\help:\universe^\length \times \b^*
\to \b^*$ used by a {\em prover} (henceforth, $P$) and a data stream algorithm
run by a {\em verifier}, $V$. Prover $P$ provides $\help(\bx,r_P)$ as
annotation to be read by $V$.  We think of $\help$ as being decomposed into
$(\help_1,\ldots,\help_{\length})$, where the function
$\help_i:\universe^{\length}\to\b^*$ specifies the annotation supplied to $V$
after the arrival of the $i$th token $x_i$. That is, $\help$ acts on
$\bx$ (using $r_P$) to create an {\em annotated stream} $\bx^\rhelp$ defined as follows:
\[
  \bx^{\rhelp} :=
  (x_1,\, \help_1(\bx,r_P),\,
    x_2,\, \help_2(\bx,r_P),\, \ldots,\,
    x_{\length},\, \help_{\length}(\bx,r_P)) \, .
\]
Note that this is a stream over $\universe \cup \b$, of length $\length +
\sum_i |\help_i(\bx,r_P)|$.  The streaming verifier $V$, who uses $w$ bits of
working memory and has oracle access to a (private) random string $r_V$, then
processes this annotated stream, eventually giving an output
$\out{V}{\bx^{\rhelp},r_V}$.

% For ease of exposition, as well as consistency with the literature on interactive proofs,
% we will regularly refer to the help function $\help$ as a \emph{prover}, which we denote by $P$.
% Likewise, we will refer to the data stream algorithm $V$ as the \emph{verifier}.

\paragraph{Prescient \aSchemes.}
%

The \ascheme\ $\alg = (\help,V)$ is said to be $\delta_s$-sound and
$\delta_c$-complete for the function $\fn$ if the following conditions hold:
\begin{enumerate}
  \item For all $\bx\in\universe^\length$, we have $\Pr_{r_P,
  r_V}[\out{V}{\bx^{\rhelp},r_V} \neq \fn(\bx)] \le \delta_c$.
  \item For all $\bx\in\universe^\length$, $\help'=(\help_1', \help_2',
  \ldots, \help_\length') \in (\b^*)^\length $, we have
    $\Pr_{r_V}[\out{V}{\bx^{\help'},r_V} \not\in \{\fn(\bx)\} \cup\{\fail\}] \le \delta_s$.
\end{enumerate}
If $\delta_c=0$, the \ascheme\ satisfies \emph{perfect completeness};
otherwise it has \emph{imperfect completeness}. An output of ``$\fail$''
indicates that $V$ rejects $P$'s claims in trying to convince $V$ to output a
particular value for $\fn(\bx)$.  

We note two important things. First, the definition of a scheme allows the
annotation $\help_{i}(\bx,r_P)$ to depend on the entire stream $\bx$, thus
modeling {\em prescience}: the advice from the prover can depend on data which
the verifier has not seen yet.  Second, $P$ must convince $V$ of the value of
$\fn(\bx)$ {\em for all} $\bx$.  This is stricter than the traditional
definitions of interactive proofs and MA communication complexity (including
our own, above) for decision problems, which place different requirements on
the cases $\fn(\bx) = 0$ and $\fn(\bx) = 1$.  In Section \ref{full::sec:graphs}, we
briefly consider a relaxed definition of schemes that is in the spirit of the
traditional definition.

We define $\err(\alg)$ to be the minimum value of $\max\{\delta_s, \delta_c\}$
such that the above conditions are satisfied. We define the {\em annotation
length} $\hcost(\alg) = \max_{\bx, r_P} \sum_i |\help_{i}(\bx,r_P)|$, the
total size of $P$'s communications, and the {\em verification space cost}
$\vcost(\alg) = w$, the space used by the verifier $V$.  We say that $\alg$ is
a \pscheme{(\anncost, c_v)} if $\hcost(\alg) = O(\anncost)$, $\vcost(\alg) =
O(c_v)$ and $\err(\alg) \le \frac13$.

\paragraph{Online \aSchemes.}
%
We call $\alg = (\help,V)$ a $\delta$-error online scheme for $\fn$ if, in
addition to the conditions in the previous definition, each function $\help_i$
depends only on $(x_1, \ldots, x_i)$.  We define error, hcost, and vcost as
above and say that $\alg$ is an {\em \oscheme{(\anncost, c_v)}} if
$\hcost(\alg) = O(\anncost)$, $\vcost(\alg) = O(c_v)$, and $\err(\alg) \le
\frac13$.

Unlike prior work \cite{full::icalp}, we do not always assume that the universe size
$n$ and stream length $\length$ are polynomially related; it is possible that
$\log \length = o(\log n)$.  Therefore we must be much more careful about
logarithmic factors than in prior work.  We do assume that $\length < n$
always, because our focus is on sparse streams.

Notice that the help function can be made deterministic in a prescient scheme,
but not necessarily so in an online scheme. This is directly analogous to the
situation for MA and online MA communication models, as discussed at the end
of Section~\ref{full::sec:communicationmodel}.

